From Hamiltonians to complex symplectic transformations

Gaussian unitaries are specified by a second order polynomial in the bosonic operators, that is, by a quadratic polynomial and a linear term. From the Hamiltonian other equivalent representations of the Gaussian unitaries are obtained, such as Bogoliubov and real symplectic transformations. The paper develops an alternative representation, called complex symplectic transformation, which is more compact and is comprehensive of both Bogoliubov and real symplectic transformations. Moreover, it has other advantages. One of the main results of the theory, not available in the literature, is that the final displacement is not simply given by the linear part of the Hamiltonian, but depends also on the quadratic part. In particular, it is shown that by combining squeezing and rotation, it is possible to achieve a final displacement with an arbitrary amount.

==> DD/CS176.tex <==
\def\BH{{\bf H}}
\def\Bh{{\bf h}}
\def\BS{{\bf S}}
\def\Bs{{\bf s}}
\unit=0.50mm \where=2 %\xF=20 \xD=45
\Z=1 \ZZ=2
\yF=4 \r=100
\poniombre
\Blocchi 
TIPO:\a=12\b=12\c=6\d=10   
DIDASCALIA:
Above the two transformations needed for the interpretation of  the affine trasformation
   $\E^{\I H}\,\xi\,\E^{-\I H^*}=\E^{-\I\,\Omega H}\;\xi+\Bs$ as
    the cascade of two transformations. Below the two eqivalent cascades. In both cascades the transformation $ \C(S)_{\B(H)}(\xi)=
 \E^{-\I\,\Omega\,\B(H)}\, \xi$ is the same, while the  displacement amounts
 are related as $\Bs=\BS \,x$. 
DOMINI:
FUNZIONI:\xi,\BS\;\xi,\BS\;\xi+\Bs, \xi,\xi+x,\BS\;\xi+\Bs,
\xi ,\BS\;\xi,\xi, \xi+x,
SCRITTE:S_{\B(H)}(\cdot),\C(D)_\Bs(\cdot),\labore,
\C(D)_{x}(\cdot),S_{\B(H)}(\cdot),
\A(20;55), S_{\B(H)}(\cdot),\A(120;55),\C(D)_x(\cdot),
SOPRASCRITTE:,,,,,,\scritta(3)(quadratic\\Hamiltonian),,
            \scritta(3)(linear\\Hamiltonian),
AGGIUNTE:\w(222,67)[1, \C(D)_x(\xi)=\E^{-\xi^*\,\Omega\,x}]
\w(60,33)[12,first interpretation] 
\w(200,33)[12,second interpretation]
FINE


==> DD/DD133.tex <==
% File: ./DD/DD133.tex creato da tipo.m il {2017, 3, 17, 18, 1, 55.342491}
\l=125  \r=51 \where=2  \unit=1.mm  
\Figura
DIDASCALIA:The displacement  amount $|s|$ as a function of $r$ and $\theta$ 
            for $h=1$. 
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(22.000,1.300){\psfig{figure=./DD/DD133s.eps ,height=50.000mm,width= 80.000mm } }
%\griglietta(12,5)
\rotw(65,2)(-2)[1,\theta]
\rotw(89.5,24)(2)[1,r]
 \EP} 
 FINE


==> DD/DD188.tex <==
% File: ./DD/DD188.tex creato da tipo.m il {2017, 3, 17, 19, 21, 24.684179}
\l=125  \r=40  \unit=1.mm  
\Figura
DIDASCALIA:Plot of $P(\phi)$ (aperiodic) and $P_0(\phi)$ (periodic)  
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(0.000,1.300){\psfig{figure=./DD/DD188A.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DD188B.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DD188B.eps ,height=40.000mm,width= 60.000mm } }
  %\griglietta(13,5)
\w(25,43)[1,|P(\phi)|]
\w(95,43)[1,|P_0(\phi)|]
\w(54,1)[1,\phi]\w(125,1)[1,\phi]
\put(21.2,-2){\Blue{\line(0,1){40}}}
\put(38.9,-2){\Blue{\line(0,1){40}}}
\put(93.5,-2){\Blue{\line(0,1){40}}}
\put(111.2,-2){\Blue{\line(0,1){40}}}
\quota(30,0)(2,c,8.4){period}
\quota(102.4,0)(2,c,8.4){period}
 \EP} 
 FINE


==> DD/DD189.tex <==
% File: ./DD/DD189.tex creato da tipo.m il {2017, 3, 17, 7, 10, 37.925072}
\l=125  \r=45  \unit=1.mm  \yF=2
\Figura
DIDASCALIA:Plot of $P(\phi)$ (aperiodic) and $P_0(\phi)$ (periodic)  
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(0.000,1.300){\psfig{figure=./DD/DD189A.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DD189B.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DD189B.eps ,height=40.000mm,width= 60.000mm } }
  %\griglietta(13,5)
\w(25,44)[1,|P(\phi)|]
\w(95,44)[1,|P_0(\phi)|]
\w(54,1)[1,\phi]\w(125,1)[1,\phi]
\put(20,-2){\Blue{\line(0,1){40}}}
\put(40,-2){\Blue{\line(0,1){40}}}
\put(110.8,-2){\Blue{\line(0,1){40}}}
\put(93,-2){\Blue{\line(0,1){40}}}
\quota(103,0)(2,c,10){period}
\quota(30,0)(2,c,10){period}
 \EP} 
 FINE


==> DD/DD190.tex <==
% File: ./DD/DD190.tex creato da tipo.m il {2017, 3, 17, 19, 26, 42.998063}
\l=125  \r=40  \unit=1.mm  
\Figura
DIDASCALIA:The displacement amount $|s|$  (left) as a function of $r$
for 6 values of $\theta$ and $h=1$ and   (right) as a function of $\theta$
for 6 values of $r$ and $h=1$
in the squeezing +displacement 
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(0.000,1.300){\psfig{figure=./DD/DD190A.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DD190B.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DD190B.eps ,height=40.000mm,width= 60.000mm } }
%\griglietta(13,5)
\w(125,1)[11,{$\to \theta$}]
 \w(70,40)[11,{\large$\uparrow$}]
  \w(67,40)[11,{$|s|$}]
  \w(135,31.6)[2,r=0.1]
  \w(135,27.8)[2,r=0.5]
  \w(135,23.4)[2,r=1]
  \w(135,19.4)[2,r=1.5]
  \w(135,15.8)[2,r=2]
  \w(135,11.5)[2,r=2.5]
  %
  \w(55,1)[11,$\to r$]
 \w(-6,40)[1,\uparrow]
  \w(-3,40)[11,{ $|s|$}]
  \w(62.5,31.5)[2,\theta=0]
  \w(62.5,27.6)[2,\theta=\pi/6]
  \w(62.5,23.5)[2,\theta=\pi/4]
  \w(62.5,19)[2,\theta=\pi/2]
  \w(62.5,15)[2,\theta=\pi]
  \w(62.5,11.0)[2,\theta=3\pi/2]
  
 \EP} 
 FINE


==> DD/DD192.tex <==
% File: ./DD/DD192.tex creato da tipo.m il {2017, 3, 17, 19, 45, 30.315490}
\l=125  \r=54  \unit=0.8mm  \where=2
\Figura
DIDASCALIA:The displacement amount $|s|$ as a function of $\theta$
and $\phi$ 
 for $h=1$ and $r=0.1$.  
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(12.000,4.300){\psfig{figure=./DD/DD192As.eps ,height=40.000mm,width= 80.000mm } }
%\put(12.000,1.300){\psfig{figure=./DD/DD192Bs.eps ,height=40.000mm,width= %80.000mm } }
%\griglietta(13,9)
          % \w(100,105)[1,r=0.1]
 \EP} 
 FINE


==> DD/DD4025.tex <==
% File: ./DE/DE4026.tex creato da tipo.m il {2016, 12, 13, 9, 9, 51.380769}
\l=125  \r=51 \where=2  \unit=0.8mm  
\Figura
DIDASCALIA:(Left) The minimum and the maximum of the displacement amount $|s|$
            as a function of $r$ obtained for $\theta=\pi$ and $\theta=0$,
	    respectively. (Right) Regions of attenuation and amplifcation of the dispacement amount
in the case of  squeezing only
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(-22.000,1.300){\psfig{figure=./DD/DE4026.eps ,height=40.000mm,width= 64.000mm } } 
\put(72.000,1.300){\psfig{figure=./DD/DE4029.eps ,height=40.000mm,width= 64.000mm } } 
 \EP} %\griglietta(12,5)
          \rotw(108,30)(40)[12,amplification]
	   \rotw(86,14)(40)[12,attenuation]
	\w(60,2)[1,r]   \w(143,2)[1,r]\w(70,50)[1,\theta]
 FINE


==> DD/DD5.tex <==



\l=125  \r=55 \yF=-3\where=2  \unit=0.8mm  
\Figura
DIDASCALIA:The  class of Gaussian unitaries with the subclasses
of displacement, rotation, and squeezing.   
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(22.000,1.300){\psfig{figure=./DD/DD5.eps ,height=40.000mm,width= 64.000mm } }  %50 80
%\griglietta(12,6)
         \w(47,39)[10,$D(\alpha)$]\w(47,30)[11,displacement]
	 \w(77,39)[10,$R(\phi)$]\w(77,30)[11,rotation]
	 \w(64.5,17)[10,$Z(z)$]\w(64.5,9)[11,squeezing]
	 \w(62,59)[11,{\bf Gaussian unitaries}] 
	   \put(62,56){\vector(0,-1){6}}
			        \EP} 
 FINE
 


==> DD/DD66.tex <==
\def\BH{{\bf H}}
\def\Bh{{\bf h}}
 \def\C(#1){{\cal #1}}
 \def\BS{{\bf S}}
\def\Bs{{\bf s}}

\def\poni{(\C(U)_E,\C(U)_E,\C(U)_F,\C(W)_E,\C(W)_F)}
 \where=2                                                
 \unit=0.7mm
 \l=120 \r=70  \yF=-4 \xF=0
%\grigliatrue 
 \Figura
 DIDASCALIA:Specifications of Gaussian unitaries and connections.
 INIZIO
\Assi0(0.000,0.000) AM=0.2  A=120.500  BM=0.000  B=90.040
inizio 
{\Thicklines
   %\put(17,20){\Red{\ellipse{10}{7}}}
   \put(25,20){\ellipse{50}{25}}  %FU
   \put(25,60){\ellipse{50}{25}}  %Ham
   \put(95,20){\ellipse{50}{25}}   %Bug 
   \put(95,60){\ellipse{50}{25}}
  \w(25,64)[11,Hamiltonian] \w(25,57.0)[1,(\BH\vl\Bh)]
  \w(95,64.0)[11,Bogoliubov] \w(95,57)[1,(E,F,s)]
  \w(25,24.0)[11,complex symplectic] \w(25,17.0)[1, (\BS\vl\Bs)]
   \w(93,24.0)[11,real symplectic]\w(95,17)[1,(\BS_0\vl \Bs_0)]
   %\put(50,60){\line(1,0){20}}
   \put(50,60){\vector(1,0){20}}
  % \put(50,20){\line(1,0){20}}
   \put(50,20){\vector(1,0){20}}
   %\put(25,47.5){\line(0,-1){14}}
   \put(25,47.5){\vector(0,-1){14.8}}
   \put(95,47.5){\vector(0,-1){14.8}}%\put(95,47){\vector(0,-1){13}}
   %\put(0,0,27){\path(45,27)(80,50)}
   \vet(45.5,27)(80,50)
  }
 fine 
 FINE


==> DD/DE189.tex <==
% File: ./DE/DE188.tex creato da tipo.m il {2017, 3, 9, 10, 27, 5.896561}
\l=125  \r=50  \unit=1.mm  
\Figura
DIDASCALIA:Plot of $P(\phi)$ (aperiodic) and $P_0(\phi)$ (periodic)  
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(0.000,1.300){\psfig{figure=./DD/DE188A.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DE188B.eps ,height=40.000mm,width= 60.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DE188B.eps ,height=40.000mm,width= 60.000mm } }
  %\griglietta(13,5)
\w(25,42)[1,|P(\phi)|]
\w(95,42)[1,|P_0(\phi)|]
\w(54,1)[1,\phi]\w(125,1)[1,\phi]
\put(110.8,-2){\Red{\line(0,1){40}}}
\put(93,-2){\Red{\line(0,1){40}}}
\w(102,0)[12,period $(-\pi,\pi)$]
 \EP} 
 FINE


==> DD/DE4010.tex <==
% File: ./DE/DE4010.tex creato da tipo.m il {2016, 12, 18, 7, 21, 44.086822}
\l=125  \r=51 \where=2  \unit=1.mm  
\Figura
DIDASCALIA:  The displacement amount $|s|$ as a function of $\theta$
 for $h=1$ , $\phi=0.5$, and for four values of $r$
in the general case  of single mode    
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(22.000,1.300){\psfig{figure=./DD/DE4010.eps ,height=50.000mm,width= 80.000mm } }
%\griglietta(12,5)
\w(96,3)[1,\to\theta]
 \w(20,50)[1,\uparrow]
  \w(17,50)[1,|s|]

  \W(101,35)[1,l,\phi=0.5]
  \W(101,29)[1,l,\phi=0.5]
  \W(101,24)[1,l,\phi=0.5]
  \W(101,19)[1,l,\phi=0.5]
%  
  \W(116,35)[1,l,r=0.5]
  \W(116,29)[1,l,r=1.0]
  \W(116,24)[1,l,r=1.2]
  \W(116,19)[1,l,r=1.4]
  
 \EP} 
 FINE


==> DD/DE4013.tex <==
% File: ./DE/DE4013.tex creato da tipo.m il {2016, 12, 15, 7, 44, 33.210879}
\l=125  \r=51 \where=2  \unit=1.mm  
\Figura
DIDASCALIA:  The displacement amount $|s|$ as a function of $\theta$
 for $h=1$  and for four values of $r$
in the  case  of  squeezing only.    
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(22.000,1.300){\psfig{figure=./DD/DE4013.eps ,height=50.000mm,width= 80.000mm } }
%\griglietta(12,5)
\w(96,3)[1,\to\theta]
 \w(20,50)[1,\uparrow]
  \w(17,50)[1,|s|]

%  
  \W(102,35)[1,l,r=0.5]
  \W(102,29)[1,l,r=1.0]
  \W(102,24)[1,l,r=1.5]
  \W(102,19)[1,l,r=2.0]
  \put(25,15){\line(1,0){65}}
  
 \EP} 
 FINE


==> DD/DE4014.tex <==
% File: ./DE/DE4014.tex creato da tipo.m il {2016, 12, 12, 7, 42, 13.109066}
\l=125  \r=92  \unit=0.8mm  \where=2
\Figura
DIDASCALIA:The displacement amount $|s|$ as a function of $\phi$
 for $h=1$ 
for different ranges of $\phi$ 
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(-2.000,50.000){\psfig{figure=./DD/DE4014A.eps ,height=32.000mm,width= 48.000mm } }
\put(72.000,50.000){\psfig{figure=./DD/DE4014B.eps ,height=32.000mm,width= 48.000mm } }
\put(-2.000,1.300){\psfig{figure=./DD/DE4014C.eps ,height=32.000mm,width= 48.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DE4014D.eps ,height=32.000mm,width= 48.000mm } }
%\griglietta(13,10)
           \w(6,40)[1,|s|]
	   \w(81,40)[1,|s|]
	   \w(6,90)[1,|s|]
	   \w(81,90)[1,|s|]
	   \w(58,0)[1,\phi]\w(133,0)[1,\phi]
	    \w(58,48)[1,\phi]\w(133,48)[1,\phi]
	    \w(45,40)[1,r=0.5\q\theta=0.5]
	     \w(130,40)[1,r=0.5\q\theta=0.5]
	    \w(45,86)[1,r=0.5\q\theta=0.5]
	     \w(130,86)[1,r=0.5\q\theta=0.5]
 \EP} 
 FINE


==> DD/DE4025.tex <==
% File: ./DE/DE4026.tex creato da tipo.m il {2016, 12, 13, 9, 9, 51.380769}
\l=125  \r=51 \where=2  \unit=0.8mm  
\Figura
DIDASCALIA:The minimum and the maximum of the displacement amount $|s|$
            as a function of $r$ obtained for $\theta=\pi$ and $\theta=0$,
	    respectively.  
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(-22.000,1.300){\psfig{figure=./DD/DE4026.eps ,height=40.000mm,width= 64.000mm } }
\put(0.00,0.00){\BP(0.00,0.00) 
\put(42.000,1.300){\psfig{figure=./DD/DE4026.eps ,height=40.000mm,width= 64.000mm } }
%\griglietta(12,5)
           \w(106,4)[1,r]
 \EP} 
 FINE


==> DD/DE4026.tex <==
% File: ./DE/DE4026.tex creato da tipo.m il {2016, 12, 13, 9, 9, 51.380769}
\l=125  \r=51 \where=2  \unit=0.8mm  
\Figura
DIDASCALIA:The minimum and the maximum of the displacement amount $|s|$
            as a function of $r$ obtained for $\theta=\pi$ and $\theta=0$,
	    respectively.  
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(22.000,1.300){\psfig{figure=./DD/DE4026.eps ,height=40.000mm,width= 64.000mm } }
%\griglietta(12,5)
           \w(106,4)[1,r]
 \EP} 
 FINE


==> DD/DE4033.tex <==
% File: ./DE/DE4033.tex creato da tipo.m il {2016, 12, 15, 17, 57, 24.410373}
\l=125  \r=92  \unit=0.8mm  \where=2
\Figura
DIDASCALIA:(nuova versione di DE4014 con formule brevi)The displacement amount $|s|$ as a function of $\phi$
           for $h=1$ 
for  ranges of $\phi$ around the divergensies points. 
INIZIO
 \put(0.00,0.00){\BP(0.00,0.00) 
\put(-2.000,50.000){\psfig{figure=./DD/DE4033A.eps ,height=32.000mm,width= 48.000mm } }
\put(72.000,50.000){\psfig{figure=./DD/DE4033B.eps ,height=32.000mm,width= 48.000mm } }
\put(-2.000,1.300){\psfig{figure=./DD/DE4033C.eps ,height=32.000mm,width= 48.000mm } }
\put(72.000,1.300){\psfig{figure=./DD/DE4033D.eps ,height=32.000mm,width= 48.000mm } }
%\griglietta(13,10)
           \w(6,40)[1,|s|]
	   \w(81,40)[1,|s|]
	   \w(6,90)[1,|s|]
	   \w(81,90)[1,|s|]
	   \w(58,0)[1,\phi]\w(133,0)[1,\phi]
	    \w(58,48)[1,\phi]\w(133,48)[1,\phi]
	    \w(45,40)[1,r=0.5\q\theta=0.5]
	     \w(130,40)[1,r=0.5\q\theta=0.5]
	    \w(45,86)[1,r=0.5\q\theta=0.5]
	     \w(130,86)[1,r=0.5\q\theta=0.5]
 \EP} 
 FINE

